Terrain-Adaptive, ALIP-Based Bipedal Locomotion Controller via Model Predictive Control and Virtual Constraints

This paper presents a gait controller for bipedal robots to achieve highly agile walking over various terrains given local slope and friction cone information. Without these considerations, untimely impacts can cause a robot to trip and inadequate tangential reaction forces at the stance foot can cause slippages. We address these challenges by combining, in a novel manner, a model based on an Angular Momentum Linear Inverted Pendulum (ALIP) and a Model Predictive Control (MPC) foot placement planner that is executed by the method of virtual constraints. The process starts with abstracting from the full dynamics of a Cassie 3D bipedal robot, an exact low-dimensional representation of its center of mass dynamics, parameterized by angular momentum. Under a piecewise planar terrain assumption and the elimination of terms for the angular momentum about the robot's center of mass, the centroidal dynamics about the contact point become linear and have dimension four. Importantly, we include the intra-step dynamics at uniformly-spaced intervals in the MPC formulation so that realistic workspace constraints on the robot's evolution can be imposed from step-to-step. The output of the low-dimensional MPC controller is directly implemented on a high-dimensional Cassie robot through the method of virtual constraints. In experiments, we validate the performance of our control strategy for the robot on a variety of surfaces with varied inclinations and textures.

==> Sections/Archive.tex <==
\section{MPC Formulation for Foot Placement Control of 3D-LIP} \label{Sec:MPC_Formulation}
The following optimization problem is summarized as an N-step receding horizon problem with quadratic cost and linear constraints as shown in \ref{eq:mpc}

\begin{equation} \label{eq:mpc}
\begin{split}
    &\min_{\mathbf{U}_{fp}} J = \sum_{k= 0}^{N_k-1} \mathbf{x}_{e,k}^T Q_k \mathbf{x}_{e,k} + \mathbf{x}_{e,N}^T Q_T \mathbf{x}_{e,N} \\
    &\mathbf{subject\ to} \\
    & \mathbf{x}_0 = \text{estimated state at end of current step} \\
    & \mathbf{x}_{e,k} = \mathbf{x}_k - \mathbf{x}^{des}, \\
    &\mathbf{x}_{k+1} = \begin{cases}
        A (\mathbf{x}_k + B \mathbf{u}_{fp,k}) & ,k \in \mathcal{K}_p \\
        A \mathbf{x}_k & ,\texttt{otherwise}
    \end{cases}, \\
    &\mathcal{K}_p = \{k:\ k = \tfrac{n T_p}{\Delta t_{disc}},\ \forall n = 1,..., N_{steps}\} \\
    &\forall\ \mathbf{x}_k \in \mathcal{X}, \\
    &\forall\ \mathbf{u}_{fp,k} \in \mathcal{U}
\end{split}
\end{equation}
The solution returns the desired foot placement vector emanating from the current stance foot to the new desired ending swing foot location (as shown in \ref{fig:2d_lip}). The initial condition, $\mathbf{x}_0$ is the estimated state of the LIP model at the end of the current step just before impact. The prediction is computed using \eqref{lip_dyn_simple} where $T$ is now the amount of time remaining. The discrete dynamics of \eqref{eq:lip_dyn_simple} and foot placement input are embedded in the equality constraints. The control input, $u_{fp}$, is only applied when $k \in \mathcal{K}_p$ where $N_{steps}$ is the step prediction horizon, $T_p$ is the step period and $\Delta t_{disc}$ is the discretization resolution of the dynamics. The sets $\mathcal{X}$ and $\mathcal{U}$ limit the states and control inputs. 

\subsection{Intra-step Dynamics}
The priority of \eqref{eq:mpc} is to compute optimal foot placements such that the robot converges to a desired periodic state. A simple formulation might omit the states throughout the transient of the step since they are uncontrollable through foot placement. since they are uncontrollable throughout the step transient. We, however, have taken special care to include the intra-step dynamics such that additional constraints on mechanical and environmental restrictions can be applied.
\noindent \textbf{Remark:} While we are not exploiting this capability here, in the next iteration we will have a gait library of virtual constraints available to the control and we will be to index into the linearized virtual constraints and impose more precise imitations on the kinematics and dynamics of individual joints and links. By using the VCs, we are able to predict forward the full dynamics of the robot as the MPC process predicts forward the dynamics of the ALIP.

\subsection{Constraint Sets}
The state constraint set $\mathcal{X}$ is the union of the mechanical safety set $\mathcal{X}^{mech}$ and the ground friction comfort set $\mathcal{X}^{slip}$. The mechanical safety set is composed on box constraints related to the geometrical limitations of the robot. The $y_c$ components of these constraints are modified based on which leg is contact with the ground in order to avoid leg collisions.

The slip constraint is computed using the 3D-LIP dynamics as a simplified approximation. In this model, the ground reaction force is applied collinearly through the contact leg since the point mass moves parallel to the ground height. Taking advantage of the known slope of the terrain we can derive the resultant tangent and normal forces with respect to the ground for both x and y components \eqref{eq:GRF_rotate}.
\begin{equation} \label{eq:GRF_rotate}
    \begin{bmatrix}
        F_{T_x} \\ F_{N_x} \\ F_{T_y} \\ F_{N_y}
        \end{bmatrix} =\begin{bmatrix}
        \cos \alpha_x & 0 & -\sin \alpha_x \\ 
        \sin \alpha_x & 0 & \cos \alpha_x \\
        0 & \cos \alpha_y & -\sin \alpha_y\\ 
        0 & \sin \alpha_y & \cos \alpha_y
        \end{bmatrix} \begin{bmatrix}
        F_x \\ F_y \\ F_z
        \end{bmatrix}
\end{equation}

From the motion constraints we can also derive the relative force ratios
\begin{equation} \label{GRF ratios}
    \begin{split}
        F_{x/z} &= \dfrac{F_x}{F_z} = \dfrac{x_c}{k_x x_c + k_y y_c + z_H} \\
        F_{y/z} &= \dfrac{F_y}{F_z} = \dfrac{y_c}{k_x x_c + k_y y_c + z_H} \\
    \end{split}
\end{equation}
% \yg{$F_z$ is not constant $mg$ when there is a slope. We might use ratio instead of exact value$F_x = \frac{x_c}{zH}F_z$}
% \GG{Good point will fix and give solution with assumptions that either ky~0 or kx~0}
We combine this with a Coulomb static friction constraint ($F_{T_{x}} \leq \mu F_{N_{x}}$) between the component tangent and normal vectors to compute the $x_c^{slip}$ and $y_c^{slip}$ constraints.
\begin{equation} \label{eq:slip}
    \begin{split}
        (1 - \mu \tan \alpha_x) F_{x/z} \ &\leq  \tan \alpha_x + \mu \\
        (1 - \mu \tan \alpha_y) F_{y/z} \ &\leq  \tan \alpha_y + \mu
    \end{split}
\end{equation}
For known $k_x$, $k_y$, and $\mu$, a conditional set of linear inequalities in $x_c$ and $y_c$ can be implemented. For simple cases of pure forward and sideways walking the inequalities simplify to 
\begin{equation} \label{eq:slip_limit_simple}
\begin{split}
    x_c &\leq \tfrac{(\mu + k_x)z_H}{1-\mu k_x} \\
    y_c &\leq \tfrac{(\mu + k_x)z_H}{1-\mu k_x} 
\end{split}
\end{equation}
Clearly, this is not an exact friction slip constraint due to the simplifications of using the 3D-LIP for ground reaction force estimation. However, it can be combined with an under-approximation of the friction coefficient $\mu$ to enable safer foot placements.

\subsection{Cost Design}
The cost function is the sum of a running cost and a terminal cost with respect to the state error at the end of each predicted step. In other words, $Q_k = \mathbf{0}, \forall k \notin \mathcal{K}_p$. Given a desired longitudinal angular momentum $L^{y,des}$ and step width $W$, we can use the expanded solutions of \eqref{eq:lip_dyn} to compute the desired state of the corresponding periodic orbit.
\begin{equation} \label{eq:lip_dyn_expand}
    \begin{split}
    x_c(T_p) &= \cosh(\ell T_p) x_c (0) + \frac{1}{m z_H \ell} \sinh(\ell T_p) L^y(0) \\
    y_c(T_p) &= \cosh(\ell T_p) y_c(0) - \frac{1}{m z_H \ell} \sinh(\ell T_p) L^x(0) \\
    L^x(T_p) &= - m H \ell \sinh(\ell T_p) y_c(0) + \cosh(\ell T_p) L^x(0) \\
    L^y(T_p) &= m z_H \ell \sinh(\ell T_p) x_c(0) + \cosh(\ell T_p) L^y(0) 
    \end{split}
\end{equation}
With the assumption of conservation of angular momentum about the contact point, we substitute $L^{y,des} = L^y(0) = L^y(T_p)$, $L^x(0) = -L^x(T_p)$, and $y_c(0) = \nicefrac{W}{2}$ into \eqref{eq:lip_dyn_expand} and solve the resultant linear system of equations.
\begin{equation}
\begin{split}
    x_c^{des} &= x_c(T_p) = \frac{1}{m z_H \ell} \tanh(\nicefrac{\ell T_p}{2}) L_y^{des} \\
    y_c^{des} &= \frac{1}{2}\text{sgn(stance)} W \\
    L^{x,des} &= - \frac{1}{2} \text{sgn(stance)}  m H \ell W \tanh(\nicefrac{\ell T_p}{2}) + L^{x,offset}
\end{split}
\end{equation}
where sgn(stance) is +1 or -1 for left stance or right stance, respectively. Here, an offset is added to $L^{x,des}$ angular momentum in order to account for lateral movment.

The terminal cost $Q_f$ is computed as the optimal cost-to-go by solving the Discrete-Time Ricatti Equation for the system in \eqref{eq:lip_with_ufp} with $T_r = T_p$. This selection of the terminal cost ensures recursive feasibility through the logic of Bellman's principle of optimality \cite{borrelli2017_LMPC}.

An interesting fact is that the foot placement solution computed by Gong \textit{et al.} can be recovered through slight modification of \eqref{eq:mpc}. By removing the cost function and constraints and appending a terminal constraint on the desired angular momentum at the end of the next step a feasibility problem can be solved to reproduce the same result.
